PKind: A parallel k-induction based model checker

PKind is a novel parallel k-induction-based model checker of invariant properties for finite- or infinite-state Lustre programs. Its architecture, which is strictly message-based, is designed to minimize synchronization delays and easily accommodate the incorporation of incremental invariant generators to enhance basic k-induction. We describe PKind's functionality and main features, and present experimental evidence that PKind significantly speeds up the verification of safety properties and, due to incremental invariant generation, also considerably increases the number of provable ones.

==> eptcsdata.tex <==
\providecommand{\firstpage}{55}
\providecommand{\publicationstatus}{Jiri Barnat and Keijo Heljanko (Eds.)\\ 10th International Workshop on\\ Parallel and Distributed Methods in verifiCation (PDMC 2011)\\
EPTCS 72, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.72.6}{10.4204/EPTCS.72.6}}
\pdfoutput=1

